Enhanced path sampling using subtrajectory Monte Carlo moves

Path sampling allows the study of rare events like chemical reactions, nucleation and protein folding via a Monte Carlo (MC) exploration in path space. Instead of configuration points, this method samples short molecular dynamics (MD) trajectories with specific start- and end-conditions. As in configuration MC, its efficiency highly depends on the types of MC moves. Since the last two decades, the central MC move for path sampling has been the so-called shooting move in which a perturbed phase point of the old path is propagated backward and forward in time to generate a new path. Recently, we proposed the subtrajectory moves, stone-skipping (SS) and web-throwing (WT), that are demonstrably more efficient. However, the one-step crossing requirement makes them somewhat more difficult to implement in combination with external MD programs or when the order parameter determination is expensive. In this article, we present strategies to address the issue. The most generic solution is a new member of subtrajectory moves, wire fencing (WF), that is less thrifty than the SS, but more versatile. This makes it easier to link path sampling codes with external MD packages and provides a practical solution for cases where the calculation of the order parameter is expensive or not a simple function of geometry. We demonstrate the WF move in a double well Langevin model, a thin film breaking transition based on classical force fields, and a smaller ruthenium redox reaction at the ab initio level in which the order parameter explicitly depends on the electron density.

==> Figures/1-hole/1-OP_vs_dt/op_vs_dt.tex <==
\begin{tikzpicture}
\begin{axis}[
xlabel={Time [ps]},
ylabel={Order parameter},
legend cell align={left},
legend entries={$\lambda_\mathrm{A/B}$,$\lambda_\mathrm{cap}$,$\lambda_\mathrm{i}$},
legend style={
draw=none,
legend pos=north west,
font=\small}]
\addplot [solid, ultra thick] coordinates {(0,5)(68,5)};
\addplot [loosely dashdotdotted, ultra thick] coordinates {(0,15)(68,15)};
\addplot [dashed, ultra thick] coordinates {(0,10)(68,10)};
\addplot [solid, ultra thick] coordinates {(0,200)(68,200)};
\addplot [purple, ultra thick] table {Figures/1-hole/1-OP_vs_dt/327-ll.txt};
\addplot [teal, ultra thick] table {Figures/1-hole/1-OP_vs_dt/329-lr.txt};
\addplot [magenta, ultra thick] table {Figures/1-hole/1-OP_vs_dt/272-lr.txt};
\addplot [blue, ultra thick] table {Figures/1-hole/1-OP_vs_dt/54-ll.txt};
\end{axis}
\node at (rel axis cs:-0.065,1.05)  {\large\textbf{a)}};
\end{tikzpicture}
